Pursuit Winning Strategies for Reach-Avoid Games with Polygonal Obstacles

This paper studies a multiplayer reach-avoid differential game in the presence of general polygonal obstacles that block the players' motions. The pursuers cooperate to protect a convex region from the evaders who try to reach the region. We propose a multiplayer onsite and close-to-goal (MOCG) pursuit strategy that can tell and achieve an increasing lower bound on the number of guaranteed defeated evaders. This pursuit strategy fuses the subgame outcomes for multiple pursuers against one evader with hierarchical optimal task allocation in the receding-horizon manner. To determine the qualitative subgame outcomes that who is the game winner, we construct three pursuit winning regions and strategies under which the pursuers guarantee to win against the evader, regardless of the unknown evader strategy. First, we utilize the expanded Apollonius circles and propose the onsite pursuit winning that achieves the capture in finite time. Second, we introduce convex goal-covering polygons (GCPs) and propose the close-to-goal pursuit winning for the pursuers whose visibility region contains the whole protected region, and the goal-visible property will be preserved afterwards. Third, we employ Euclidean shortest paths (ESPs) and construct a pursuit winning region and strategy for the non-goal-visible pursuers, where the pursuers are firstly steered to positions with goal visibility along ESPs. In each horizon, the hierarchical optimal task allocation maximizes the number of defeated evaders and consists of four sequential matchings: capture, enhanced, non-dominated and closest matchings. Numerical examples are presented to illustrate the results.

==> dominance_regions.tex <==
\section{Dominance Regions}

==> isochrones.tex <==
\section{Isochrones}

\begin{thom}[Isochrones under PLS obstacles]
cc
\end{thom}


==> winning_regions.tex <==
\section{Winning Regions}

==> winning_strategy.tex <==
\section{Winning strategy}

The positions of the pursuer $P$ and the evader $E$ are $\bm{x}_P$ and $\bm{x}_E$, and their initial positions are $\bm{x}_{P0}$ and $\bm{x}_{E0}$. Let $\mathbb{E}(t)$ be the evasion region at time $t$ and $\mathbb{C}$ be the region after expanding the initial evasion region with size $\delta>0$. For capture radius $r \ge 0$, if $\| \bm{x}_P - \bm{x}_E \|_2 \ge r$, then define the potential function $f : \mathbb{R}^2 \times \mathbb{R}^2 \times \mathbb{R}^2 \to \mathbb{R}$:
\begin{equation}\label{eq:defi-f}
    f(\bm{x}, \bm{x}_P, \bm{x}_E) = \| \bm{x} - \bm{x}_P \|_2 - \alpha \| \bm{x} - \bm{x}_E \|_2 - r
\end{equation}
for $\bm{x} \in \mathbb{R}^2$, where $\alpha > 1$ is the speed ratio. For $\mathbb{C}$, we define the potential function $f : \mathbb{R}^2 \to \mathbb{R}$:
\begin{equation}
    g(\bm{y}) = \| \bm{y} - \bm{x}_{P0} \|_2 - \alpha \| \bm{y} - \bm{x}_{E0} \|_2 - r + \delta
\end{equation}
for $\bm{y} \in \mathbb{R}^2$ such that $\mathbb{C} = \{ \bm{y} \in \mathbb{R}^2 \mid g(\bm{y}) \ge 0 \}$.

At time $t$, we denote by $d_{\textup{min}}(t)$ and $d_{\textup{max}}(t)$ be the minimum and maximum distances between $\mathbb{E}(t)$ and $\partial \mathbb{C}$, respectively. Therefore,
\begin{equation}\label{eq:d-min}
\begin{aligned}
   d_{\textup{min}}(t) = & \underset{(\bm{x},\bm{y})\in\mathbb{R}^2\times\mathbb{R}^2}{\textup{minimize}}
	&& \rho (\bm{x}, \bm{y}) \\
	&\textup{ subject to}&& f(\bm{x},\bm{x}_P, \bm{x}_E) \ge 0 \\
 & & & g(\bm{y}) \leq 0
\end{aligned}
\end{equation}
and 
\begin{equation}\label{eq:d-max}
\begin{aligned}
   d_{\textup{max}}(t) = & \underset{(\bm{x},\bm{y})\in\mathbb{R}^2\times\mathbb{R}^2}{\textup{maximize}}
	&& \rho (\bm{x}, \bm{y}) \\
	&\textup{ subject to}&& f(\bm{x},\bm{x}_P, \bm{x}_E) \leq 0, \, g(\bm{x}) \ge 0 \\
 & & & f(\bm{y},\bm{x}_P, \bm{x}_E) \leq 0, \, g(\bm{y}) \ge 0\,.
\end{aligned}
\end{equation}

If $(\bm{x}_{\textup{min}}^\star, \bm{y}_{\textup{min}}^\star)$ is the optimal solution to \eqref{eq:d-min}, then by KKT condition we have
\begin{subequations}\label{eq:kkt-condition-min}
\begin{align}
	&\bm{0}= \rho_{\bm{x}} (\bm{x}_{\textup{min}}^\star, \bm{y}_{\textup{min}}^\star) + \lambda_1 f_{\bm{x}} (\bm{x}_{\textup{min}}^\star, \bm{x}_P, \bm{x}_E) \label{itm:min-KKT-1}\\
	&\bm{0}= \rho_{\bm{y}} (\bm{x}_{\textup{min}}^\star, \bm{y}_{\textup{min}}^\star) + \lambda_2 g_{\bm{y}} (\bm{y}_{\textup{min}}^\star) \label{itm:min-KKT-2}\\
	& f(\bm{x}_{\textup{min}}^\star, \bm{x}_P, \bm{x}_E) \ge 0, \lambda_1 \leq 0, \lambda_1 f(\bm{x}_{\textup{min}}^\star, \bm{x}_P, \bm{x}_E) = 0 \label{itm:min-KKT-3}\\
	&g(\bm{y}_{\textup{min}}^\star) \leq 0, \lambda_2 \ge 0, \lambda_2 g(\bm{y}_{\textup{min}}^\star) = 0 \label{itm:min-KKT-4}
\end{align}
\end{subequations}
and $d_{\textup{min}}(t) =  \rho (\bm{x}_{\textup{min}}^\star, \bm{y}_{\textup{min}}^\star)$. Additionally, since $\bm{x}_{\textup{min}}^\star$ and $\bm{y}_{\textup{min}}^\star$ are at the boundaries of $\mathbb{E}(t)$ and $\mathbb{C}$ all the time respectively, i.e., $f (\bm{x}_{\textup{min}}^\star, \bm{x}_P, \bm{x}_E) \equiv 0$ and $g (\bm{y}_{\textup{min}}^\star) \equiv 0$, then 
\begin{equation*}
    \dod{f (\bm{x}_{\textup{min}}^\star, \bm{x}_P, \bm{x}_E)}{t} = 0, \quad \dod{g (\bm{y}_{\textup{min}}^\star)}{t} = 0
\end{equation*}
and thus letting $f^{\textup{min}} \coloneqq f(\bm{x}_{\textup{min}}^\star, \bm{x}_P, \bm{x}_E) $, $g^{\textup{min}}  \coloneqq g(\bm{y}_{\textup{min}}^\star)$, we have
\begin{equation} \label{eq:from-state-to-control-min}
\begin{aligned}
    f_{\bm{x}}^{\textup{min}\top} \dot{\bm{x}}_{\textup{min}}^\star = - f_{\bm{x}_P}^{\textup{min}\top} \dot{\bm{x}}_P - f_{\bm{x}_E}^{\textup{min}\top} \dot{\bm{x}}_E, \,
    g_{\bm{y}}^{\textup{min}\top} \dot{\bm{y}}_{\textup{min}}^\star = 0 \,.
\end{aligned}
\end{equation}

Similarly, if $(\bm{x}_{\textup{max}}^\star, \bm{y}_{\textup{max}}^\star)$ is the optimal solution to \eqref{eq:d-max}, by KKT condition we have
\begin{equation*}
 \begin{aligned}
	& \bm{0}=  - \rho_{\bm{x}} (\bm{x}_{\textup{max}}^\star, \bm{y}_{\textup{max}}^\star) + \lambda_3 f_{\bm{x}} (\bm{x}_{\textup{max}}^\star, \bm{x}_P, \bm{x}_E) + \lambda_4 g_{\bm{y}}(\bm{x}_{\textup{max}}^\star) \\
	&\bm{0}=  - \rho_{\bm{y}} (\bm{x}_{\textup{max}}^\star, \bm{y}_{\textup{max}}^\star) + \lambda_5 f_{\bm{x}} (\bm{y}_{\textup{max}}^\star, \bm{x}_P, \bm{x}_E) + \lambda_6 g_{\bm{y}}(\bm{y}_{\textup{max}}^\star)  \\
	& f(\bm{x}_{\textup{max}}^\star, \bm{x}_P, \bm{x}_E) \leq 0, \lambda_3 \ge 0, \lambda_3 f(\bm{x}_{\textup{max}}^\star, \bm{x}_P, \bm{x}_E) = 0 \\
	&g(\bm{x}_{\textup{max}}^\star) \ge 0, \lambda_4 \leq 0, \lambda_4 g(\bm{x}_{\textup{max}}^\star) = 0 \\
 	& f(\bm{y}_{\textup{max}}^\star, \bm{x}_P, \bm{x}_E) \leq 0, \lambda_5 \ge 0, \lambda_5 f(\bm{y}_{\textup{max}}^\star, \bm{x}_P, \bm{x}_E) = 0 \\
	&g(\bm{y}_{\textup{max}}^\star) \ge 0, \lambda_6 \leq 0, \lambda_6 g(\bm{y}_{\textup{max}}^\star) = 0
\end{aligned}   
\end{equation*}
and $d_{\textup{max}}(t) =\rho (\bm{x}_{\textup{max}}^\star, \bm{y}_{\textup{max}}^\star)$. since $\bm{x}_{\textup{min}}^\star$ and $\bm{y}_{\textup{min}}^\star$ are at the boundaries of $\mathbb{E}(t)$ and $\mathbb{C}$ all the time respectively


To simplify the notation, we take $f^{\textup{min}} \coloneqq f(\bm{x}_{\textup{min}}^\star, \bm{x}_P, \bm{x}_E) $, $g^{\textup{min}}  \coloneqq g(\bm{y}_{\textup{min}}^\star)$, $f^{\textup{max}} \coloneqq f(\bm{x}_{\textup{max}}^\star, \bm{x}_P, \bm{x}_E) $ and $g^{\textup{max}}  \coloneqq g(\bm{y}_{\textup{max}}^\star)$.

We consider the Lyapunov-like function 
\begin{align}
    V(t) = d_{\textup{min}}(t) d_{\textup{max}}(t) \,.
\end{align}
If $d_{\textup{min}}(t) > 0$ for all $t \ge 0$, then we can conclude that the evason region $\mathbb{E}(t)$ remains within $\mathbb{C}$ all the time. Initially, $V(0) > 0$ because by construction $\mathbb{C}$ is an expanding region of $\mathbb{E}(0)$. We consider the time derivative of $V$ as follows:
\begin{equation} \label{eq:v-dot-1}
\begin{aligned}
    \dot{V}(t) & = \dot{d}_{\textup{min}} d_{\textup{max}} + d_{\textup{min}} \dot{d}_{\textup{max}} \\
    & = (\rho_{\bm{x}}^\top (\bm{x}_{\textup{min}}^\star, \bm{y}_{\textup{min}}^\star) \dot{\bm{x}}_{\textup{min}}^\star + \rho_{\bm{y}}^\top (\bm{x}_{\textup{min}}^\star, \bm{y}_{\textup{min}}^\star) \dot{\bm{y}}_{\textup{min}}^\star) d_{\textup{max}} \\
    & \quad +  (\rho_{\bm{x}}^\top (\bm{x}_{\textup{max}}^\star, \bm{y}_{\textup{max}}^\star) \dot{\bm{x}}_{\textup{max}}^\star + \rho_{\bm{y}}^\top (\bm{x}_{\textup{max}}^\star, \bm{y}_{\textup{max}}^\star) \dot{\bm{y}}_{\textup{max}}^\star) d_{\textup{min}} \\
    & = - (\lambda_1 f_{\bm{x}}^{\textup{min}\top} \dot{\bm{x}}_{\textup{min}}^\star + \lambda_2 g_{\bm{y}}^{\textup{min}\top} \dot{\bm{y}}_{\textup{min}}^\star ) d_{\textup{max}} \\
    & \quad + (\lambda_3 f_{\bm{x}}^{\textup{max}\top} \dot{\bm{x}}_{\textup{max}}^\star + \lambda_4 g_{\bm{y}}^{\textup{max}\top} \dot{\bm{y}}_{\textup{max}}^\star ) d_{\textup{min}}.
\end{aligned}
\end{equation}
For $\bm{x}_{\textup{max}}^\star$ and $\bm{y}_{\textup{max}}^\star$, the same argument leads to
\begin{equation} \label{eq:from-state-to-control-max}
\begin{aligned}
    f_{\bm{x}}^{\textup{max}\top} \dot{\bm{x}}_{\textup{max}}^\star = & - f_{\bm{x}_P}^{\textup{max}\top} \dot{\bm{x}}_P - f_{\bm{x}_E}^{\textup{max}\top} \dot{\bm{x}}_E \\
    g_{\bm{y}}^{\textup{max}\top} \dot{\bm{y}}_{\textup{max}}^\star = & \ 0 \,.
\end{aligned}
\end{equation}
Then, by \eqref{eq:from-state-to-control-min} and \eqref{eq:from-state-to-control-max}, $\dot{V}(t)$ satisfies the lower bound
\begin{equation}
\begin{aligned}
   \dot{V}(t)  = \ & \lambda_1 (f_{\bm{x}_P}^{\textup{min}\top} \dot{\bm{x}}_P + f_{\bm{x}_E}^{\textup{min}\top} \dot{\bm{x}}_E) d_{\textup{max}} \\
   & - \lambda_3 (f_{\bm{x}_P}^{\textup{max}\top} \dot{\bm{x}}_P + f_{\bm{x}_E}^{\textup{max}\top} \dot{\bm{x}}_E ) d_{\textup{min}}
   \\
   = \ & (\lambda_1 d_{\textup{max}} f_{\bm{x}_P}^{\textup{min}} - \lambda_3 d_{\textup{min}} f_{\bm{x}_P}^{\textup{max}})^\top \dot{\bm{x}}_P \\
    & + (\lambda_1 d_{\textup{max}} f_{\bm{x}_E}^{\textup{min}} - \lambda_3 d_{\textup{min}} f_{\bm{x}_E}^{\textup{max}})^\top \dot{\bm{x}}_E \ge p_1 - p_2
\end{aligned}
\end{equation}
where $p_1 \coloneqq v_P\| \lambda_1 d_{\textup{max}} f_{\bm{x}_P}^{\textup{min}} - \lambda_3 d_{\textup{min}} f_{\bm{x}_P}^{\textup{max}} \|_2$ and $p_2 \coloneqq v_E \| \lambda_1 d_{\textup{max}} f_{\bm{x}_E}^{\textup{min}} - \lambda_3 d_{\textup{min}} f_{\bm{x}_E}^{\textup{max}} \|_2$. Using \eqref{eq:defi-f}, four partial derivatives in $p_1$ and $p_2$ meet the following conditions
\begin{equation}
\begin{aligned}
    f_{\bm{x}_P}^{\textup{min}} f_{\bm{x}_P}^{\textup{max}} & = \cos \angle \bm{x}_{\textup{min}}^\star \bm{x}_P \bm{x}_{\textup{max}}^\star \\
    f_{\bm{x}_E}^{\textup{min}} f_{\bm{x}_E}^{\textup{max}} & = \alpha^2 \cos \angle \bm{x}_{\textup{min}}^\star \bm{x}_E \bm{x}_{\textup{max}}^\star.
\end{aligned}
\end{equation}
Letting $\ell_{P1} = \| \bm{x}_{\textup{min}}^\star - \bm{x}_P \|_2$, $\ell_{P2} = \| \bm{x}_{\textup{max}}^\star - \bm{x}_P \|_2$, $\ell_{E1} = \| \bm{x}_{\textup{min}}^\star - \bm{x}_E \|_2$, $\ell_{E2} = \| \bm{x}_{\textup{max}}^\star - \bm{x}_E \|_2$ and $\ell_0 = \| \bm{x}_{\textup{min}}^\star - \bm{x}_{\textup{max}}^\star\|_2$, then
\begin{equation*}
\begin{aligned}
    & \cos \angle \bm{x}_{\textup{min}}^\star \bm{x}_E \bm{x}_{\textup{max}}^\star - \cos \angle \bm{x}_{\textup{min}}^\star \bm{x}_P \bm{x}_{\textup{max}}^\star \\
    & =  \frac{\ell_{E1}^2 + \ell_{E2}^2 - \ell_0^2  }{2 \ell_{E1} \ell_{E2}} - \frac{\ell_{P1}^2 + \ell_{P2}^2 - \ell_0^2  }{2 \ell_{P1} \ell_{P2}} \\
    & = \frac{\ell_{E1}^2 + \ell_{E2}^2 - \ell_0^2  }{2 \ell_{E1} \ell_{E2}} - \frac{(\alpha \ell_{E1} + r )^2 + (\alpha \ell_{E2} + r)^2 - \ell_0^2  }{2 (\alpha \ell_{E1} + r) (\alpha \ell_{E2} + r)} \\
    & = \frac{(r^2 + \alpha r (\ell_{E1} + \ell_{E2})) ((\ell_{E1} - \ell_{E2})^2 - \ell_0^2)}{2 \ell_{E1} \ell_{E2} (\alpha \ell_{E1} + r) (\alpha \ell_{E2} + r) } \\
    & \quad + \frac{(1 - \alpha^2) \ell_0^2 \ell_{E1} \ell_{E2}}{2 \ell_{E1} \ell_{E2} (\alpha \ell_{E1} + r) (\alpha \ell_{E2} + r) } \\
    & \leq \frac{(1 - \alpha^2) \ell_0^2 }{2 (\alpha \ell_{E1} + r) (\alpha \ell_{E2} + r) }
\end{aligned}
\end{equation*}

$p_1^2 - p_2^2$ has the lower bound
\begin{equation}
\begin{aligned}
    p_1^2 - p_2^2  & = 2 v_P^2 \lambda_1 \lambda_3 d_{\textup{min}} d_{\textup{max}} (f_{\bm{x}_E}^{\textup{min}} f_{\bm{x}_E}^{\textup{max}} - f_{\bm{x}_P}^{\textup{min}} f_{\bm{x}_P}^{\textup{max}}) \\
    & =  2 v_P^2 \lambda_1 \lambda_3 d_{\textup{min}} d_{\textup{max}} (\cos \angle \bm{x}_{\textup{min}}^\star \bm{x}_E \bm{y}_{\textup{min}}^\star - \cos \angle \bm{x}_{\textup{min}}^\star \bm{x}_P \bm{y}_{\textup{min}}^\star) 
\end{aligned}
\end{equation}

